LOCALINTEL: Generating Organizational Threat Intelligence from Global and Local Cyber Knowledge

Security Operations Center (SoC) analysts gather threat reports from openly accessible global threat repositories and tailor the information to their organization's needs, such as developing threat intelligence and security policies. They also depend on organizational internal repositories, which act as private local knowledge database. These local knowledge databases store credible cyber intelligence, critical operational and infrastructure details. SoCs undertake a manual labor-intensive task of utilizing these global threat repositories and local knowledge databases to create both organization-specific threat intelligence and mitigation policies. Recently, Large Language Models (LLMs) have shown the capability to process diverse knowledge sources efficiently. We leverage this ability to automate this organization-specific threat intelligence generation. We present LocalIntel, a novel automated threat intelligence contextualization framework that retrieves zero-day vulnerability reports from the global threat repositories and uses its local knowledge database to determine implications and mitigation strategies to alert and assist the SoC analyst. LocalIntel comprises two key phases: knowledge retrieval and contextualization. Quantitative and qualitative assessment has shown effectiveness in generating up to 93% accurate organizational threat intelligence with 64% inter-rater agreement.

==> qualitative_table.tex <==

\begin{table}
\caption{Fleiss Multirater Kappa Analysis: Substantial agreement (approx. 0.65) among three raters evaluating 60 scenarios on the basis of \emph{correctness}.} \label{tab:felis}
 %\vspace{-1mm}
  % \begin{minipage}{0.5\linewidth}
    %\centering
    
    
    {\renewcommand{\arraystretch}{1.3}%
\footnotesize

\begin{tabular}{ll|l} 
\hline
                                    & \multicolumn{2}{l}{\textbf{Overall Categories $^ {a,b}$}}  \\ \cline{1-3}
\multirow{2}{*}{Overall Agreement}  & Kappa  ($K$)             & Standard Error        \\ \cline{2-3}
                                    & \cellcolor{green!15} 0.6476841         & 0.076706           \\ \cline{1-3}
\multicolumn{3}{l}{a. Data contains 60 scenario and ground truth pairs evaluated by 3 raters using Fleiss Kappa.} \\
\multicolumn{3}{l}{b. Rating category values are case-sensitive.}              
\end{tabular}
% \end{minipage}

}

\end{table}
